Lossy Image Compression with Quantized Hierarchical VAEs

Recent research has shown a strong theoretical connection between variational autoencoders (VAEs) and the rate-distortion theory. Motivated by this, we consider the problem of lossy image compression from the perspective of generative modeling. Starting with ResNet VAEs, which are originally designed for data (image) distribution modeling, we redesign their latent variable model using a quantization-aware posterior and prior, enabling easy quantization and entropy coding at test time. Along with improved neural network architecture, we present a powerful and efficient model that outperforms previous methods on natural image lossy compression. Our model compresses images in a coarse-to-fine fashion and supports parallel encoding and decoding, leading to fast execution on GPUs. Code is available at https://github.com/duanzhiihao/lossy-vae.

==> sections/deprecated-background.tex <==

\subsection{Variational AutoEncoders}
% Let $\mathbf{x}$ representing the data with an underlying (unknown) distribution $p_\text{data}(\cdot)$, and let $x$ be the observed samples drawn from it. VAEs posit a parameterized joint distribution $p_{\mathbf{x},\mathbf{z}}(x,z) = p_{\mathbf{x}|\mathbf{z}}(x|z) p_{\mathbf{z}}(z)$, where
Let $\mathbf{x}$ represent the observed variable with an underlying (unknown) distribution $p_\text{data}(\cdot)$. Variational autoencoders (VAEs) posit a joint distribution $p_{X,Z}(x,z) = p_{X|Z}(x|z) p_Z(z)$ parameterized by $\theta$. As $p_{Z|X}(\cdot)$ is intractable to compute, VAE also learns an approximate posterior $q_\phi(\mathbf{z}|\mathbf{x})$.
For each data point $x$, the training objective is to minimize the variational upper bound on the negative log-likelihood (NLL):
% \begin{equation}
% \mathcal{L}_{\theta, \phi}(x) = D_{\text{KL}}(q_\phi(\mathbf{z}|\mathbf{x}=x) \parallel p_\theta(\mathbf{z})) + 
%                                 \mathbb{E}_{\mathbf{z} \sim q_\phi(\mathbf{z}|\mathbf{x}=x)}\left[ \log \frac{1}{p_\theta(x | \mathbf{z})} \right].
% \end{equation}
\begin{equation}
\label{eq:nelbo}
\mathcal{L}_\text{NELBO}(x) = D_{\text{KL}}(q_{Z|X=x} \parallel p_Z)
                 + \mathbb{E}_{Z \sim q_{Z|X=x}}\left[ \log \frac{1}{p_{X|Z}(x | Z)} \right].
\end{equation}
% The $\beta$-VAE~\citep{higgins2016betavae} has the following form:
% \begin{equation}
% \mathcal{L}_{\theta, \phi}(x) = D_{\text{KL}}(q_\phi(\mathbf{z}|\mathbf{x}=x) \parallel p_\theta(\mathbf{z})) + 
%                                 \mathbb{E}_{\mathbf{z} \sim q_\phi(\mathbf{z}|\mathbf{x}=x)}\left[ D(x, f(\mathbf{z})) \right].
% \end{equation}
% \begin{equation}
% \mathcal{L}(x) = D_{\text{KL}}(q_{Z|X=x} \parallel p_Z)
%                  + \mathbb{E}_{Z \sim q_{Z|X=x}}\left[ d(f(Z), x) \right].
% \end{equation}




\subsection{Relationship to Rate Distortion Theory}
From rate distortion theory~\cite{cover2005information}, we know that the minimum achievable rate $R(D)$ with distortion $D$ is given by the (information) rate distortion function:
\begin{equation}
R(D) = \min_{E[d(\hat{X}, X)] < D} I(X;\hat{X}).
\end{equation}
The rate distortion function typically does not have a closed form for complex sources such as images.
\cite{yang2022sandwich} has shown that a modified version of negative ELBO is a tight upper bound on the rate distortion function.
\begin{equation}
\mathcal{L}(x) = D_{\text{KL}}(q_{Z|X=x} \parallel p_Z)
                 + \lambda \mathbb{E}_{Z \sim q_{Z|X=x}}\left[ d(f(Z), x) \right].
\end{equation}


% \begin{equation}
% \begin{aligned}
%     \mathcal{L}
%     &= \mathbb{E}_{\mathbf{z} \sim q_\phi(\mathbf{z}|\mathbf{x}=x)} \left[
%         \log \frac{p_\theta(x, \mathbf{z})}{q_\phi(\mathbf{z} | x)}
%     \right].
%     \\
%     &= \mathbb{E}_{\mathbf{z} \sim q_\phi(\mathbf{z}|\mathbf{x}=x)} \left[
%         \log \frac{1}{q_\phi(\mathbf{z} | x)} - \log \frac{1}{p_\theta(x, \mathbf{z})}
%     \right].
% \end{aligned}
% \end{equation}




